Multi-Robot Motion Planning for Unit Discs with Revolving Areas

We study the problem of motion planning for a collection of $n$ labeled unit disc robots in a polygonal environment. We assume that the robots have revolving areas around their start and final positions: that each start and each final is contained in a radius $2$ disc lying in the free space, not necessarily concentric with the start or final position, which is free from other start or final positions. This assumption allows a weakly-monotone motion plan, in which robots move according to an ordering as follows: during the turn of a robot $R$ in the ordering, it moves fully from its start to final position, while other robots do not leave their revolving areas. As $R$ passes through a revolving area, a robot $R'$ that is inside this area may move within the revolving area to avoid a collision. Notwithstanding the existence of a motion plan, we show that minimizing the total traveled distance in this setting, specifically even when the motion plan is restricted to be weakly-monotone, is APX-hard, ruling out any polynomial-time $(1+\epsilon)$-approximation algorithm. On the positive side, we present the first constant-factor approximation algorithm for computing a feasible weakly-monotone motion plan. The total distance traveled by the robots is within an $O(1)$ factor of that of the optimal motion plan, which need not be weakly monotone. Our algorithm extends to an online setting in which the polygonal environment is fixed but the initial and final positions of robots are specified in an online manner. Finally, we observe that the overhead in the overall cost that we add while editing the paths to avoid robot-robot collision can vary significantly depending on the ordering we chose. Finding the best ordering in this respect is known to be NP-hard, and we provide a polynomial time $O(\log n \log \log n)$-approximation algorithm for this problem.

==> old/algorithm-old.tex <==
\paragraph*{Retracting a robot $\mathbf{B_j}$.}
When $R_i$ is active, $R_j$ is at the location $z_j$. 
We define the \emph{retraction function} $\rho_{ij}$. 
Since $i$ is fixed, for simplicity we set $\rho_j \coloneqq \rho_{ij}$. 
If the center of $R_i$ is at distance at least $2$ from $z_j$, then $R_i$ does not intersect $D_{z_j}$, so there is no need to move $R_j$ from $z_j$. 
Therefore we set $\rho_{j}(p) = z_j$ for all $p$ such that $\norm{p - z_j} \geq 2$. 
On the other hand $\overline{\gamma_i}$ does not intersect the interior of $F_{z_j}$ so $\rho_j(p)$ is undefined for $p \in \interior(F_{z_j})$. 
We thus focus on the case when $\norm{p - z_j} \leq 2$, in which case $p \in B_{z_j}$, and $p \not \in \interior(F_{z_j})$. 
Hence, assume that $p \in B_{z_j} \setminus F_{z_j}$. 
Let $D^+(p)$ be the disk of radius $2$ centered at $p$. 
Note that for a point $q \in \reals^2$, $D_p \cap D_q \neq \emptyset$ if and only if $q \in D^+(p)$. 
Intuitively, we move $R_j$ from $z_j$ (such that its center still lies in $C_{z_j}$ as little as possible so that $R_j$ does not collide with $R_i$ if $R_i$ is at point $p$. 

% There are two cases for retraction: 

% % replaced.. 
% Let the robot moving from its start to target position be the \emph{active} robot, and its path be the \emph{active path}. 
% As a robot moves from its start to target position, other robots only move within their revolving area to avoid collisions between the active robot and other robots. 

% Since our goal is to minimize the total length of paths, one natural set of paths to consider is the shortest paths from $s_i$ to $t_i$ which avoids obstacles. 
% However, these paths might collide with other robots. 
% Rather than treat other robots as obstacles, we can utilize revolving areas to move non-active robots out of the way of shortest paths. 
% In this way, our algorithm need only make small edits to the initial set of shortest paths.  
% Indeed, we will show this intuitive idea gives rise to a constant approximation algorithm. 


% First, the algorithm finds a set of paths $\Gamma = \{\gamma_1,...,\gamma_n\}$ lying in $\mathsf{F}$, where
% $\gamma_i : [0,1] \rightarrow \mathsf{F}$ is a path from $s_i$ to $t_i$, avoiding obstacles but ignoring possible collisions with other robots. 
% Then, the algorithm modifies $\Gamma$ in order to avoid collisions between the robots. 
% Specifically, let $\sigma$ be an arbitrary ordering of $1, 2, \dots, n$. 
% The algorithm iterates over the paths in order defined by $\sigma$, and based on each $\gamma_{\sigma(i)}$, it defines a new $\pi_{\sigma(i)}$ so that $\pi_{\sigma(i)}$ does not pass through the core $A^{in}_z$ of an occupied revolving area. 
% Additionally, we show that we can define \emph{retraction paths} for non-active robots-- paths within their respective revolving areas, defined in a manner that avoids collision with the active robot. 

% In Section~\ref{sec:retration}, we define the retraction paths and prove they result in a feasible set of paths. 
% In Section~\ref{sec:approximation}, we show that if $\Gamma$ is a set of shortest paths, the edits to $\Pi$ along with the retraction path lengths do not increase the cost by more than a constant factor: $\ell(\Pi) = O(1) \ell(\Gamma)$, and therefore $\ell(\Pi) = O(1) \ell(\Pi^*)$, where $\Pi^*$ is an optimal set of paths.

% \paragraph*{Path Deformation.}
% For simplicity, we assume robots move in order $1, 2, \dots, n$, and that robot $i$ is the active robot in the time interval $[i-1, i]$. This means that robots $1, \dots, i-1$ are in their target positions and robots $i+1, \dots, n$ are in their start positions. 
% Thus, when considering $\pi_i$ we only need to focus on the $n-1$ occupied revolving areas. 
% Let the occupied revolving areas during time $[i-1, i]$ be $Z_i \subseteq S \cup T$. 

% Given a set $\Gamma$ of initial paths, we edit path $\gamma_i$ when a portion of $\gamma_i$ lies inside the core of a revolving area in $Z_i$. 
% Suppose $\gamma_i \cap A^{in}_j \neq \emptyset$.
% We edit path $\gamma_i$ to instead only lie on $\partial A^{in}_j$ (the same technique described in~\cite{solomon2018motion}). 
% For any $z \in Z_i$, consider any entrance point $p = \gamma_i(t)$ such that $p \in A^{in}_z$ and $\gamma_{i}(t-\eps) \not \in A^{in}_z$, and any exit point $q = \gamma_i(t)$ such that $q \in A^{in}_z$ and $\gamma_i(t+\eps) \not \in A^{in}_z$, for infinitesimally small $\eps > 0$.
% Sort these intersection points by their order of appearence in $\gamma_i$. 
% Remove the portion of $\gamma_i$ between a $p, q$ entrance, exit pair and replace it with the geodesic arc of $\partial A^{in}_z$ from $p$ to $q$. 
% Repeat this process for every intersection point with the core $A^{in}_z$ and all revolving areas in $Z_i$. 
% The new path is free from collision with obstacles and does not intersect any $A^{in}_z$ for $z \in Z_i$.
% Let the set of deformed paths be $\Pi$. 
% We next show that we can define retraction paths for non-active disks for each path in $\Pi$.  

% \section{Retraction Paths}
% \label{sec:retration}
% Suppose robot $i$ is active, and consider point $p \in \pi_i$. 
% For each robot $j \neq i$, let the location of $j$ be $z_j$ (for $j = 1, \dots, i-1$, $z_j = f_j$ and for $j = i+1, \dots, n$, $z_j = s_j$. 
% For any $p$ and $z_j$ such that $d(p, z_j) > 2$, robot $j$ does not move from $z_j$ at time $t$ when disk $i$ is at point $p$. 
% Thus, we define retraction paths only when $d(p, z_j) \leq 2$ and movement is necessary to avoid collision. 

% Assume that $p \in \pi_i$ and $p \in A^{out}_j$, but $p \not \in A^{in}_j$ for some robot $j \neq i$, i.e., that $p$ lies within the outer disk of robot $j$, but does not intersect the interior of the core. 
% Note that $D(p, 2)$ represents the circle in which the center of robot $j$ cannot lie without collision as robot $i$ is centered at point $p$.
% We define a retraction point of robot $j$ with respect to $p$. 

% Let $r_j(p)$ be the retraction point of robot $j$ with respect to $p$: 
% \[ r_j(p) \coloneqq \argmin_{D(c_j, 1) \setminus D(p, 2)} \norm{q - z_j}. \] 
% \end{definition}
For a fixed $p$, let $\bar{p}$ be the point furthest from $p$ on $\partial C_z$. 
We define $\rho_j(p)$ as the intersection point between $D^+_p$ and segment $\overline{z_j \bar{p}}$. 
Note that $\rho_j(p)$ must exist as $p \not \in C_j$, additionally, $r_j(p)$ is unique. 
When $d(p, z_j) \geq 2$, $r_j(p) = z_j$, as described. 
% We describe the arc $r_j(p)$ lies on.  
% First, note that $\partial D(c_j, 1)$ and $\partial D(p, 2)$ intersect at exactly $2$ points. 
% If they were only tangent, we would not have that $p \in A^{out}_j$. 
% Additionally, $D(p, 2)$ cannot contain $D(c_j, 1)$ since $p$ must lie outside $A^{in}_j$.
% Let the two intersection points be $x_{j,1}(p)$ and $x_{j,2}(p)$. 
% % See figure~\ref{fig:cone-case}. 

% If $z_j$ lies in the sector $\mathsf{S}$ of $D(p, 2)$ defined by the points of $D(p, 2)$ lying between $\overline{px_{j1}(p)}$ and $\overline{px_{j2}(p)}$, then the retraction point $r_j(p)$ is the unique point on the ray $\overrightarrow{pz_j}$ at the point of intersection with $\partial D(p, 2)$.
% The closest point in $A^{in}_j$ from $z_j$ is on the straight line from $z_j$ to the feasible region where $j$ can lie. 
% Since $z_j$ lies inside $\mathsf{S}$, this point lies on the arc of $\partial D(p, 2)$ between points $x_{j1}(p)$ and $x_{j2}(p)$.

% \begin{figure}[t]
%     \begin{minipage}{.5\textwidth}
%     \centering
%     \includegraphics[width=0.7\linewidth]{sj-incone.pdf}
%     \caption{$s_j$ inside sector defined by $p$.}
%     \label{fig:cone-case}
%     \end{minipage}
%     \begin{minipage}{.5\linewidth}
%     \centering
%     \includegraphics[width=0.7\textwidth]{sj-outisde.pdf}
%     \caption{$s_j$ lies outside sector.}
%     \label{fig:outside-case}
%     \end{minipage}
% \end{figure}


% If $z_j$ lies outside the sector $\mathsf{S}$, the retraction point is 
% \[ \argmin_{q \in \{x_{j,1}(p), x_{j,2}(p) \}} \norm{ q - z_j }. \]
% The closest point to $z_j$ is intersection point between $\partial D(p, 2)$ and $\partial D(c_j, 1)$, since there is no point on the $pz_j$ line that lies in the feasible retraction region $A^{in}_j \setminus D(p, 2)$.
% This is exactly $x_{j,1}(p)$ or $x_{j, 2}(p)$. 
% Let $\mathsf{A}$ be the arc of $\partial D(p, 2)$ with endpoints $x_{j,1}(p)$ or $x_{j, 2}(p)$.
% We showed that the retraction point lies on arc $\mathcal{A}$.  
% Let the segment $\mathsf{S}_1$ be the segment $\overline{p x_{j, 1}(p)}$ and let $\mathsf{S}_2$ be the segment $\overline{p, x_{j, 2}(p)}$. Segments $\mathsf{S}_1$ and $\mathsf{S}_2$ define the sector $\mathcal{S}$. 

In the retraction path defined above, there is no initial movement along an entire segment $\overline{z_j \rho_{j}(p)}$ when the first intersection between the active robot and revolving area occurs as in~\cite{solomon2018motion}. 
Instead as $D^+_p$'s intersection with $C_z$ grows, the retraction point moves continuously. 
So when they first become tangent, the retraction point is $z_j$, and remains $z_j$ until necessary to move to maintain the invariant that $i$ and $j$ should not collide. 
% When $p \in$
    
We define retraction paths by moving robot $j$ to its retraction point $\rho_j(p)$ for each point $p \in \pi_i$ that lies in $B_j$.
Note that when $p \in \partial  B_j$ the retraction point $\rho_j(p) = z_j$, so robot $j$ starts and ends at $z_j$.
Also, note that all retraction points lie in $C_j$, so the robot $j$ always lies within its revolving area $A_{z_j}$.

Finally, we define the final set of paths $\Pi$ so that each $\pi_i: [0, n] \rightarrow \reals^2$. 
When $i$ is the active disk, for each $j \neq i$, the disk $j$ follows its retraction path. 
% More specifically, at each time $t$ when disk $i$ lies at $p \in \pi_i$, disk $j$ lies at $\rho_j(p)$. 
% \textcolor{red}{When following the retraction path, the non-active robot $j$ is no longer moving unit speed? In Section 2.5~\cite{solomon2018motion}, the active robot stops moving while the non-active robot moves along a segment to its retraction point, but in our setting things are described simultaneously. Maybe we should just point this out somewhere.}

\subsection{Feasibility} 
We show that by following retraction paths, there are no collisions between robots. 
In the following section, we assume that $i$ is the active robot, $p \in \pi_i$, and $p \in B_j$ but $p \not \in F_j$ for some robot $j$. 
Note that the retraction point lies on $\partial D^+_p$. Thus, we have the following observation. 

\begin{observation}
\label{obs:active-safe}
Robot $i$ and $j$ do not collide, since $\norm{r_j(p) - p} \geq 2$, by definition of the retraction region. 
\end{observation}

Thus, we only need to show that robot $i$ does not collide with another robot $k \neq i, j$ which might also be moving along a retraction path. 
We first prove that the segment $\overline{z_j c_j}$ associated with robot $j$ is separated from segments $\overline{z_k c_k}$ for robots $k \neq j$.

\begin{lemma}
\label{lem:dist-segments}
For any $j \neq k$ and $z_j, z_k \in S \cup T$, $d(\overline{c_j z_j}, \overline{c_k z_k}) \geq 2$.
\end{lemma}

\begin{proof}
Let $d$ denote the minimum Euclidean distance between two segments.
Let $y_j \in \overline{z_j c_j}$ and $y_k \in \overline{z_k c_k}$ be the two points realizing $d\left(\overline{z_j c_j}, \overline{z_k c_k}\right)$.
First, note that $\overline{z_j c_j}$ and $\overline{z_k c_k}$ are disjoint, since $\overline{z_j c_j} \in C_j$ and $\overline{z_k c_k} \in C_k$ and these disks do not intersect. 
This implies that either $y_j$ or $y_k$ will be an endpoint of their segments. 

Assume that $y_j$ is an endpoint of $\overline{z_j c_j}$ (otherwise we can swap labels). 
Recall that $\norm{c_j - z_k}, \norm{c_k - z_j} \geq 3$. 
We consider the triangle defined by $y_j$, $y_k$, and the endpoint of $\overline{z_kc_k}$ which is at least distance $3$ away from $y_j$ (if $y_j = z_j$ this is $c_k$, otherwise if $y_j = c_j$ this is $z_k$). 
The distance between $y_k$ and either endpoint of $\overline{c_k z_k}$ is at most $1$. 
Thus, by triangle inequality, $d(y_j, y_k) \geq 2$. 
\end{proof}

% \begin{figure}[t]
% \begin{minipage}{.5\textwidth}
%     \centering
%     \includegraphics[width=0.7\linewidth]{new-seg.pdf}
%     \caption{$f_j(p)$ when $s_j$ outside sector defined by $p$.}
%     \label{fig:new-segment}
% \end{minipage}
% \begin{minipage}{.5\textwidth}
%     \centering
%     \includegraphics[width=0.7\linewidth]{trig.pdf}
%     \caption{Let $A = p$, $B_1 = f_j(p)$, $C_1 = f_k(p)$, $B_2 = r_j(p)$, and $C_2 = r_k(p)$.}
%     \label{fig:triangle}
%     \end{minipage}
% \end{figure}

\begin{theorem}
\label{thm:no-collision}
For distinct disks $i, j, k$ and for path $\pi_i$ of disk $i$, robot $j$ and robot $k$ do not collide at any retraction point defined with respect to any point $p \in \pi_i$.
\end{theorem}

\begin{proof} 
This is equivalent to showing that $\norm{r_j(p) - r_k(p)} \geq 2$ for every $p \in \pi_i$. 

\paragraph*{Case 1: $r_j(p) = z_j$ or $r_k(p) = z_k$.}
In this case, at least one robot does not move from its starting point. 
A robot does not intersect any revolving area besides its own, so $A_j \cap D(z_k, 1) = \emptyset$ (resp. $A_k \cap D(z_j, 1) = \emptyset$) and $r_j(p) \in A^{in}_j$ (resp. $r_k(p) \in A^{in}_k$).
Thus, $\norm{r_j(p) - r_k(p)} \geq 2$ as desired. 

\paragraph*{Case 2: Both robot $i$ and $j$ move.}
In this case, $z_j, z_k \in D(p, 2)$. 
Let $f_j(p) = z_j$ if $z_j$ lies within the sector $\mathcal{S}$ (i.e. the retraction point lies on $A \setminus \{x_{j,1}(p), x_{j,2}(p) \}$. 
Otherwise, $z_j$ lies outside the sector and assume its retraction point is $x_{j, 1}(p)$. 
In this case, let $f_j(p)$ be the point on $\overline{px_{j,1}(p)}$ intersecting $\overline{z_j c_j}$.
This point must exist because $c_j$ lies inside sector $\mathsf{S}$ and $z_j$ lies outside.
% , see figure~\ref{fig:new-segment}.
Note that $f_j(p)$ lies on segment $\overline{p r_j(p)}$. 
Similarly define $f_k(p)$. 

In either case, $f_j(p) \in \overline{z_j c_j}$ and $f_k(p) \in \overline{z_k c_k}$. 
Therefore, Lemma~\ref{lem:dist-segments} implies that $\norm{f_j(p) - f_k(p)} \geq 2$.
Additionally, $f_j(p) \in D(p, 2)$, so $\norm{p, f_j(p)} \leq 2$ (similarly  $\norm{p, f_k(p)} \leq 2$). 

Consider the triangle formed by points $p, f_k(p)$ and $f_j(p)$. 
Let $\alpha$ be the angle defined by $\angle f_k(p) p f_j(p)$.
Since $\norm{p - f_j(p)}, \norm{p - f_k(p)} \leq 2$, and $\norm{f_j(p) - f_k(p)} \geq 2$, $\alpha \geq \pi/3$. 

Now consider $\triangle r_k(p) p r_j(p)$. 
Note that $\angle f_k(p) p f_j(p) = \angle r_k(p) p r_j (p)$. 
By definition $\abs{\overline{pr_j(p)}} = \abs{\overline{p r_k(p)}} = 2$ and $\angle p r_k(p) r_k(p) = \angle p r_j(p) r_k(p)$. 
Since $\angle r_k(p) p r_j (p) \geq \pi/3$, $\overline{r_j(p) r_k(p)}$ is the longest edge of the triangle $\triangle p r_j(p) r_k(p)$.
% see Figure~\ref{fig:triangle}. 
Therefore $\norm{r_j(p) - r_k(p)} \geq 2$, as desired.
\end{proof}

We can apply Theorem~\ref{thm:no-collision} to any two robots whose revolving areas intersect the path of the active robot. Thus, by combining Observation~\ref{obs:active-safe} and Theorem~\ref{thm:no-collision}, we see that following the retraction paths over the course of executing a set of paths $\Pi$ results in a set of collision free paths. 

\subsection{Analysis}
\label{sec:approximation}
\erin{The following analysis of cost will be changed with the new retraction.}
% \label{sec:approximation}
In this section, our goal is to bound the total length of movement by non-active robots (disks $j \neq i$ which move from $z_j$ during time $[i-1, i]$). 
We will charge the length of retraction paths to the portion of the active path $\pi_i$ which lies in the revolving area, by showing the retraction path is at most a constant times longer than the active path's intersection with a revolving area. 
Since a point of an active path can only lie in a constant number of revolving areas, a portion of an active path is charged at most a constant number of times. 
Thus, all disk movement in time $[i-1, i]$ can be charged to the active path, and the total length of movement is at most a constant factor larger than $\ell(\pi_i)$. 
We describe the charging argument in this section. 

\subsection{Retraction Path Charging} 
Let $p = (p_x, p_y)$ be a point. 
Consider an active path $\pi_i$, and a retraction path $R_j(\pi_i)$. 
Consider subpath $\varphi$ of $\pi_i$ with endpoints $p_1, p_2 \in \pi_i$ such that for $p \in \varphi$, $d(p, z_j) \leq 2$ (if $d(p, z_j) > 2$, then $R_j(p) = z_j$ and robot $j$ does not move).

There are three cases to consider: 
\begin{enumerate}
    \item $\varphi \in \partial A^{in}_j$,
    \item $\varphi \not\in \partial A^{in}_j$ and $r_j(p)$ is an endpoint of arc $\mathsf{A}$, 
    \item $\varphi \not\in \partial A^{in}_j$ and $r_j(p)$ lies on the interior of arc $\mathsf{A}$.
\end{enumerate}

We define an \textit{event} as a time when the retraction path switches between two of the above cases. 
For the latter two cases, (i.e., $\varphi$ does not lie on the boundary of the core of the revolving area), 
we make the further assumption that $\phi$ is the line segment $\overline{p_1p_2}$ and is such that $p_1 p_2$ lie below and to the left of $z_j$. 
Otherwise, We could split $\phi$ and apply the lemma to each segment (after rotation). 
We first consider cases two and three, and describe the retraction path for such that such a $\phi$. 
The next lemma shows that for $\phi$ satisfying Case $2$, the retraction path has length at most $4\norm{\phi}$. 
% We will consider each connected component of $\pi_{i, A_j}$ (so we treat each time $\pi_i$ enters and leaves $A_j$ separately.

\begin{lemma}
\label{lem:c4}
Let $\overline{p_1 p_2} \in \pi_i$ be a segment such that $r_j(p) \not \in \partial A^{in}_j$ for $p \in \overline{p_1p_2}$, and $d(p, s_j) \leq 2$. 
If $\overline{p_1 p_2} \in \pi_i$ such that $\norm{\overline{p_1p_2}} = \delta$, the retraction path of robot $j$ has length at most $4\delta$. 
\end{lemma}

% \note{Set $t^* = 1$, and let $\delta$ just be the length? The proof should go through).}
\begin{proof}
For simplicity, we assume $s_j = (0, 0)$.
Additionally, without loss of generality assume $p_1$ and $p_2$ lie below and to the left of $s_j$ such that $\overline{p_1p_2}$ is vertical (distances are invariant under rotation and reflection). 
We parameterize the path of robot $i$ and the retraction path of robot $j$ by variable $t$, and show that the length of the retraction path is at most a constant factor longer than the associated segment of $\pi_i$. 
Let $p \in \overline{p_1 p_2}$ and $q = R_j(p)$. 
We want to show there exists some constant $c$ such that 
\[ c \int_{0}^{t^*} \sqrt{\frac{dp_x}{dt}^2 + \frac{dp_y}{dt}^2} \geq \int_{0}^{t^*} \sqrt{\frac{dq_x}{dt}^2 + \frac{dq_y}{dt}^2}. \]
Or equivalently: 
\begin{equation}
\label{eq:main}
     c  \Paren{\frac{dp_x}{dt}^2 + \frac{dp_y}{dt}^2} \geq \frac{dq_x}{dt}^2 + \frac{dq_y}{dt}^2.
\end{equation}
Note that $\frac{d p_x}{dt} = 0$ since $\overline{p_1p_2}$ is rotated so that the segment is vertical. 
Let $\Paren{\frac{d p_y}{dt}}^2 = \alpha^2$ ($\alpha$ can be thought of as the rate of movement of $p$), so the left hand side of Equation~\ref{eq:main} simplifies to $c\alpha^2$. 

Consider the right triangle with hypotenuse $\overline{p z_j}$ with third point $(0, p_y)$.
Let $\theta$ be the angle by $p$ and let $d$ be the length of side $p, (0, p_y)$. 
The, $\Paren{\frac{d\theta}{dt}}^2 = \alpha^2 \cos^2 \theta$. 

In fact, the retraction path is defined from the fixed point $z_j$, the curve $\pi_i$, and length $2$, and is the known Chonchoid of Nicomedes~\textcolor{red}{(include a reference?).}
The distance from $z_j$ to $q$ is $2 - \frac{d}{\cos \theta}$. 
Letting $q = (r, \theta)$ we have, 

\[ \begin{aligned}
    \frac{dq_x}{d\theta}^2 + \frac{dq_y}{d\theta}^2 &= r^2 + \Paren{\frac{dr}{d\theta}}^2 \\ 
    &= \Paren{2 - \frac{2}{\cos \theta}} + \Paren{\frac{-d \sin \theta}{\cos^2 \theta}}^2 \\ 
    &= 4 - \frac{4d}{\cos \theta} + \frac{d^2}{\cos^2 \theta} + \frac{d^2 \tan^2 \theta}{\cos^2 \theta}\\ 
    &= 4 - \frac{4d}{\cos \theta} +  \frac{d^2}{\cos^4 \theta}. 
\end{aligned}\]

Note that $\cos \theta \geq d/2$, since $\cos \theta = \frac{d}{d(p, z_j)}$ and $d(p, z_j) < 2$. 

Thus, we have: 
\[ \begin{aligned}
\frac{dq_x}{dt}^2 + \frac{dq_y}{dt}^2 &= \Paren{\frac{dq_x}{d\theta}^2 + \frac{dq_y}{d\theta}^2} \frac{d\theta}{dt} \\
&= 4\alpha^2\cos^2 \theta- 4d\alpha^2 \cos \theta  +  \frac{d^2\alpha^2}{\cos^2 \theta}\\ 
&\leq 4\alpha^2 \cos^2 \theta - 8\alpha^2 \cos^2 \theta + 4\alpha^2 = 4\alpha^2 - 4\alpha^2 \cos^2 \theta 
\end{aligned} \] 

Now, plugging into equation~\ref{eq:main}, we have 

\[ c \alpha^2 \geq 4\alpha^2 - 4 \cos^2 \theta, \]
or $c \geq 4 - 4\cos^2 \theta \geq 4$ for the relevant domain. 
Thus, $c = 4$ is sufficient to prove the desired inequality. 
\end{proof}

    The next lemma shows that for a subpath $\phi$ satisfying Case $3$, the retraction path has length at most $\sqrt{2} \pi/2 \norm{\phi}$. 78



\begin{lemma}
\label{lem:intersect}
Suppose $\overline{p_1 p_2} \in \pi_i$ is a segment such that $R_j(p) \in \partial A^{in}_j$ and for all $p \in \overline{p_1p_2} \not \in \partial A^{in}_j$.
If $\overline{p_1 p_2} \in \pi_i$ such that $\norm{\overline{p_1p_2}} = \delta$, the retraction path of robot $j$ has length at most $\frac{\sqrt{2}\pi}{2} \delta$. 
\end{lemma}

\begin{proof}
For simplicity, we assume $p_1 = (0, 0)$, $p_2 = (0, \delta)$ and $c_j = (d, 0)$. Note that we can rotate and reflect circle $D(p_1, 2)$, $D(p_2, 2)$ and $A^{in}_j$ in order to obtain these coordinates. We think of $\delta$ as being a small positive constant (for the purposes of this proof, $\delta \leq 1$ is sufficient), so we can think of $D(p_2, 2)$ as the result of vertically translating $D(p_1, 2)$. For intersection points of $D(p_1, 2)$ and $C_j$, assume that the closest point to $z_j$ is the intersection point with the larger $y$-coordinate, the other case follows analogously. 
For small $\delta$, this implies that the closest intersection point of $D(p_1, 2)$ and $C_j$ to $z_j$ will also be the intersection point with the larger $y$-coordinate. 
% Also observe that $d = (1, 2]$ in order for the $R_j(p_1), R_j(p_2)$ to lie on  $C_j$. 
% If this is not the case, we apply the lemma with different segments. 

We can compute the intersection point of $A^{in}_j$ with both discs centered at $p_1$ and $p_2$ respectively. Let $q_1 \coloneqq R_j(p_1)$ and $q_2 \coloneqq R_j(p_2)$. The retraction path of $j$ with respect to segment $\overline{p_1p_2}$ is the arc of $A^{in}_j$ between $q_1$ and $q_2$. Consider any chord $ab$ of $A^{in}_j$. If the chord has length $d$, the corresponding smaller arc between $ab$ has length at most $\pi/2 d(a, b)$. We can see this by letting the $a$ and $b$ be two diametrically opposed points, so $d(a,b) = 2$, the diameter of $A^{in}_j$. The corresponding arc length is $\pi/2 d(a,b)$, and this placement of $a$ and $b$ maximizes the difference between the chord length and arc length. Thus, if we show $d(q_1, q_2) \leq c \delta$ for some constant $c$, we conclude that retraction path has length at most $\frac{c \pi \delta}{2}$. 

Define $c = \sqrt{\delta^2 + d^2}$ and $h = \frac{1}{4} \sqrt{(c+3)(c+1)(c-1)(3-c)}$. Finding the coordinates of $q_1$ and $q_2$ we have: 
\[ \begin{aligned}
q_1 &= \Paren{\frac{3+d^2}{2d}, \sqrt{4 -\frac{3+d^2}{2d}}}\\
q_2 &= \Paren{\frac{d}{2} + \frac{3d}{2c^2} + \frac{2\delta h}{c^2}, \frac{\delta}{2} - \frac{3\delta}{2c^2} + \frac{2 d h}{c^2}}.
\end{aligned}\]

We will show that $d(q_1, q_2) = \sqrt{(q_{2x} - q_{1x})^2 + (q_{2y} - q_{1y})^2} \leq \sqrt{2} \delta$ by showing $(q_{2x} - q_{1x})^2 \leq \delta^2$ and $(q_{2y} - q_{1y})^2 \leq \delta^2$. 

First, we show that $q_{2x} - q_{1x} \leq \delta$. 
$q_{2x} - q_{1x} = \frac{-3}{2d} + \frac{3d}{2(d^2 + \delta^2)} + \frac{2\delta h}{c^2}$. 
We will show that the first two terms are at most $0$. 
If $\frac{-3}{2d} + \frac{3d}{2(d^2 + \delta^2)} \leq 0$, this implies $\frac{d^2}{(d^2 + \delta^2)} \leq 1$, and indeed $d^2 \leq d^2 + w^2$. 
Indeed, $q_{2x} - q_{1x} \leq \frac{2\delta h}{c^2}$, and to finish we observe that $2h \leq c^2$, or equivalently $(c+3)(c+1)(c-1)(3-c) \leq 4c^4$. 
This implies $q_{2x} - q_{1x} \leq \frac{2\delta h}{c^2} \leq \delta$. 

Next, we show that $q_{2x} - q_{1x} \geq -\delta$.
We have $q_{2x} - q_{1x} = \frac{-3}{2d} + \frac{3d}{2(d^2 + \delta^2)} + \frac{2\delta h}{c^2} \geq \frac{-3}{2d} + \frac{3d}{2(d^2 + \delta^2)}$. 
Taking the derivative with respect to $\delta$, 
\[ \frac{\partial}{\partial \delta} \Paren{\frac{-3}{2d} + \frac{3d}{2(d^2 + \delta^2)}} = \frac{(3 (d^4 + 3 d^2 x^2))}{(2 x^2 (d^2 + \delta^2)^2)}. \] 
This implies the function is increasing, thus, we only consider $d = 1$.
If $\frac{-3}{2} + \frac{3}{2(1+\delta^2)} \geq -\delta$, then $\frac{3}{2} \leq \frac{3}{2(1+\delta^2)} + \delta$. Taking a derivative with respect to $\delta$ is always positive, so the right hand side is increasing, and at $\delta = 0$ the expression is indeed satisfied. 
Thus, we conclude that $q_{2x} - q_{1x} \geq -\delta$, and putting the above facts together $(q_{2x} - q_{1x})^2 \leq \delta^2$ as desired. 

Next, we consider $q_{2y} - q_{1y} = \frac{\delta}{2} - \frac{3\delta}{2c^2} + \frac{2 d h}{c^2} - \sqrt{4 -\frac{3+d^2}{2d}} \coloneqq b$. 
Consider the function $\frac{\delta}{2} - b$. We will show that $\frac{\delta}{2} - b \geq 0$, and conclude that $b \leq \delta/2 \leq \delta$ as desired. 
Taking the derivative of $(\delta/2 - b)$ shows that the expression  is increasing with respect to $\delta$.
Evaluating at $x = 0$, we have $(\delta/2 - b)\lvert_{\delta=0} = \sqrt{4- \Paren{\frac{3}{2d} + \frac{d}{2}}^2} + \frac{2h}{d} \geq \sqrt{4- \Paren{\frac{3}{2d} + \frac{d}{2}}^2}$. 
To show this is non-negative, note that $3/2d + d/2 \leq 2$ for $d \in (1, 2]$. 
Thus, we conclude $q_{2y} - q_{1y} \leq x$. 
We can prove $q_{2y} - q_{1y} \geq -x$ similarly to the previous case, considering the function $b + \delta$ and showing $b+\delta \geq 0$, which implies $b \geq -\delta$ as desired. 
% $\frac{-3}{2} + \frac{3}{2(1+\delta^2)} \geq -\delta$. 
%could do more here 
\end{proof}

Thus, we have considered both Case $2$ and $3$. 
For case $1$, $\phi$ is an arc on $\partial A^{in}_j$ and the retraction path of disk $j$ is the diametrically opposed arc of the same length along $\partial A^{in}_j$. 
Thus, in Case $1$ the retraction path has the same length as $\phi$. 

\subsection{Approximation Algorithm}

Suppose $\Gamma$ is a set of initial shortest paths, for example these can be computed in $O(n^2)$ time~\cite{hershberger1988n2}. 
We show that the final set of paths $\Pi$ computed from the initial set $\Gamma$ has cost $O(\ell(\Gamma))$. 

\paragraph*{Path Deformation.}
In Section~\ref{sec:alg}, we described the initial editing of $\Gamma$ so that each $\gamma_i$ does not intersect $C_j$ for $j \neq i$. 
This increases the cost of a path $\gamma_i$ by at most a factor of $\pi$ for any intersection $\gamma_i \cap A_j$ for a revolving area $A_j$. 
If $\pi_i$ intersected $C_j$, the length of $\pi_i$ inside revolving area $A_j$ was at least $2$: $\ell \cost(\gamma_i \cap A_j) \geq 2$, so we can charge the increase in length of the path deformation to a length $2$ segment of $\gamma_i$ intersecting $A_j$. 

\paragraph*{Simultaneous Retractions.}
For a single $p \in \pi_i$, a robot $j$ moves along a retraction path only if $\norm{p - z_j} \leq 2$. For a fixed $p \in \pi_i$, there are at most $6$ robots $j$ such that $z_j$ is within $2$ of $p$. Suppose there could be more. Let the distance from $p$ to each $z_j$ be $2$. If there more than $6$ such robots, the must be an angle formed by some $z_j, p, s_k$ which is less than $\pi/3$, which implies that $\norm{z_j - s_k} < 2$, which is not possible.
% \textcolor{blue}{Note: We should be able to improve this to $5$: if there are $6$ robots, each are exactly distance $2$ away from $p$. As soon as robot $i$ moves from $p$, one of the $6$ robots will not be within distance $2$ any longer, and therefore was not actually moving along a retraction path.} 

% \erin{The following might be better stated in a lemma? There might be more to say about integrating over all the pathlets.}

\paragraph*{Constant Approximation.}
Let $\Pi = \{ \pi_1, \dots, \pi_n\}$ be the set of paths which result from first finding the set of shortest paths $\Gamma$, then editing the paths of $\Gamma$ using the path deformation strategy and retraction path strategy defined in Section~\ref{sec:prelim} and Section~\ref{sec:retration}.
We have shown that $\Pi$ is a feasible set of paths. 

Now, we show we can bound by the cost increase of the total movement from the original cost of $\Pi$ by a constant factor.
Suppose the length of the optimal motion plan is $OPT$. Note that $\ell(\Pi) \leq OPT$, since $\Pi$ is the set of shortest paths disregarding any robot-robot interaction. 

Consider $\phi \coloneqq \pi_i \cap A_j$ for some $j$, and let $\phi_1, \dots, \phi_\tau$ be the connected components of $\phi$. 
We divide each $\phi_s$ into \textit{pathlets} defined by the events of the retraction path of disk $j$. 
Thus, whenever the retraction path switches cases described above, an event occurs and a new pathlet of $\phi_s$ begins. 
Any pathlet of $\phi_s$ is part of a shortest path defined with respect to polygonal obstacles, so consists of line segments and circular arcs. 
Additionally, each pathlet is compact, and can be approximated by infinitesimal line segments. 
Each pathlet is associated with a type of retraction: for each line segment approximating the pathlet we can apply either Lemma~\ref{lem:c4} or Lemma~\ref{lem:intersect} to show that the retraction path has length at most a constant factor more than the line segment of the pathlet. 
Integrating over the line segments approximating the pathlet shows that the retraction path has length at most $4$ times that of the length of the pathlet. 

From the initial set of paths $\Gamma$, we increase the total cost by a factor of $\pi$ from the path deformation, a factor of $4$ from the retraction paths, and a factor of $6$ from the number of retraction paths charging to the same point of the active path, therefore the total cost increase is at most a factor of $24\pi$. Therefore, we obtain the following theorem. 

\begin{theorem}
Let $W \subset \reals^2$ be a polygonal environment, and let $S$ be a set of start positions and $T$ be a set of end positions. Let $OPT$ be the optimal cost of any set of feasible paths. The algorithm described finds a set of paths $\Pi$ moving disks from positions $S$ to $T$ with length $O(OPT)$. 
\end{theorem}




% old....
% \erin{Redefining things in 
% Consider $\phi \coloneqq \pi_i \cap A_j$ for some $j$, and let $\phi_1, \dots, \phi_\tau$ be the connected components of $\phi$. 
% We divide each $\phi_s$ into \textit{pathlets} defined by the events of the retraction path of disk $j$. 
% Thus, whenever the retraction path switches cases described above, an event occurs and a new pathlet of $\phi_s$ begins. 
% Any pathlet of $\phi_s$ is part of a shortest path defined with respect to polygonal obstacles, so consists of line segments and circular arcs. 
% Additionally, each pathlet is compact, and can be approximated by infinitesimal line segments. 
% Each pathlet is associated with a type of retraction: for each line segment approximating the pathlet we can apply either Lemma~\ref{lem:c4} or Lemma~\ref{lem:intersect} to show that the retraction path has length at most a constant factor more than the line segment of the pathlet. 
% Integrating over the line segments approximating the pathlet shows that the retraction path has length at most $4$ times that of the length of the pathlet. 

% There are three two to consider: 
% \begin{enumerate}
%     \item $\varphi \not\in  W_j$ and $\rho_j(p)$ is an endpoint of arc $\partial D^+_p$, 
%     \item $\varphi \not\in W_j$ and $\rho_j(p)$ lies on the interior of arc $\partial D^+_p$.
% \end{enumerate}

% We define an \textit{event} as a time $t$ when the retraction path switches between two of the above cases. 
% For the latter two cases, (i.e., $\varphi$ does not enter $W_z$), 
% we make the further assumption that $\phi$ is the line segment $\overline{p_1p_2}$ and is such that $p_1 p_2$ lie below and to the left of $z_j$. 
% Otherwise, We could split $\phi$ and apply the lemma to each segment (after rotation). 
% We first consider cases two and three, and describe the retraction path for such a $\phi$. 
% The next lemma shows that for $\phi$ satisfying Case $2$, the retraction path has length at most $O(\ell{\phi})$. 

% \erin{In the following $p_1 p_2$ is a vertical segment such that $p_2$ is on the $x$-axis. We cannot make both assumptions at once? However for a segment $p_1 p_2$ we can use a radial segment + 


As before, we consider fixing active robot $R_i$ and path $\pi_i$ such that $\pi_i$ intersects the revolving area $A_j$ of disk and there is a point $p \in \pi_i$ such that $\norm{p - z_j} \geq 2$.
% In this section, we only consider the subset of path $\pi_w$ which does not intersect the interior of disk $W_j$. 
% Let a \emph{pathlet} be a subset of the path $\pi_i[p, q]$. 

% We first subdivide $\pi_i \cap A_j$ into pathlets. 
% For each connected component of $\pi_i \cap A_j$, we create a separate pathlet. 
% Next, for each pathlet, we subdivide it at any point where the \textit{type} of retraction point changes
% (recall that for a $p \in \pi_i$, the retraction point $\rho_j(p)$ is either type intersection or sector).
% There are only a finite number of pathlets since the shortest path $\gamma_i$ is compact.
% Finally, we subdivide pathlets if they contain points in the interior of $W_j$, and discard any pathlets $\varphi$ such that $\varphi \in \interior(W_j)$, as we handle these in the next Section~\ref{subsection:retraction-core}. 
% Let $\Phi = \{ \varphi_1, \dots, \varphi_k \}$ be the resulting set of pathlets, each associated with a type of retraction point. 
% Note that for any $p \in \varphi$, $p \not \in W_j$, so $\norm{p - z_j} \geq 1/2$. 

==> old/old-proofs.tex <==
In the following section, we assume that $R_i$ is the active robot, $p \in \pi_i$, and $p \in B_j$ but $p \not \in C_j$ for some robot $j$. 
Note that the retraction point lies on $\partial D^+_p$. Thus, we have the following observation. 

\begin{observation}
\label{obs:active-safe}
Robot $i$ and $j$ do not collide, since $\norm{r_j(p) - p} \geq 2$, by definition of the retraction region. 
\end{observation}

robot $i$ does not collide with another robot $k \neq i, j$ which might also be moving along a retraction path. 
We first prove that the segment $\overline{z_j c_j}$ associated with robot $j$ is separated from segments $\overline{z_k c_k}$ for robots $k \neq j$.

Assume without loss of generality that $y_j$ is an endpoint of $\overline{z_j c_j}$.
By Lemma~\ref{lem:ra-ppts}, $\norm{c_j - z_k}, \norm{c_k - z_j} \geq 3$. 
We consider the triangle defined by $y_j$, $y_k$, and the endpoint of $\overline{z_kc_k}$ which is at least distance $3$ away from $y_j$ (if $y_j = z_j$ this is $c_k$, otherwise if $y_j = c_j$ this is $z_k$). 
The distance between $y_k$ and either endpoint of $\overline{c_k z_k}$ is at most $1$ since they lie in a unit circle. 
Thus, by triangle inequality, $\norm{y_j - y_k} \geq 2$. 
